FROCC: Fast Random projection-based One-Class Classification

We present Fast Random projection-based One-Class Classification (FROCC), an extremely efficient method for one-class classification. Our method is based on a simple idea of transforming the training data by projecting it onto a set of random unit vectors that are chosen uniformly and independently from the unit sphere, and bounding the regions based on separation of the data. FROCC can be naturally extended with kernels. We theoretically prove that FROCC generalizes well in the sense that it is stable and has low bias. FROCC achieves up to 3.1 percent points better ROC, with 1.2--67.8x speedup in training and test times over a range of state-of-the-art benchmarks including the SVM and the deep learning based models for the OCC task.

==> sections/declaration.tex <==
\section{Declarations}
\subsection{Funding}
The authors did not receive funds, grants or support from any organization for the submitted work.
\subsection{Conflicts of interest/Competing interests}
The authors have no relevant financial or non-financial interests to disclose.
\subsection{Availability of data and material}
All data used in the submitted work is available freely and sources are cited appropriately.
\subsection{Code availability}
The code will be made available publicly upon acceptance of the paper.

==> sections/tab_time.tex <==
\begin{table}
    \resizebox{\columnwidth}{!}{
        \begin{tabular}{lcccccccc}
            \toprule
                             & OC-SVM & IsoForest     & Deep SVDD & Auto Encoder & \frocc        \\
            \midrule
            MNIST            & 11.63  & \emph{1.15}   & 137.30    & 297.78       & \textbf{0.97} \\
            Omniglot         & 21.56  & \emph{2.15}   & 195.21    & 345.45       & \textbf{1.52} \\
            CIFAR-10         & 16.74  & \emph{1.65}   & 165.12    & 320.54       & \textbf{1.33} \\
            CIFAR-100        & 15.31  & \emph{1.53}   & 148.71    & 310.49       & \textbf{1.24} \\
            GTSRB            & 15.21  & \emph{1.51}   & 139.54    & 314.31       & \textbf{1.11} \\
            MiniBooNE        & 8.23   & \textbf{0.69} & 16.43     & 25.65        & \emph{0.87}   \\
            MAGIC Telescope  & 9.54   & \textbf{0.54} & 14.36     & 21.88        & \emph{0.72}   \\
            SATLOG-Vehicle   & 10.94  & \textbf{0.81} & 21.73     & 32.32        & \emph{1.09}   \\
            Diabetes         & 0.11   & \textbf{0.06} & 1.41      & 1.21         & \emph{0.09}   \\
            Cardiotocography & 0.14   & \textbf{0.09} & 2.21      & 1.48         & \emph{0.12}   \\
            \bottomrule
        \end{tabular}
    }
    \caption{Training time (s) for baselines and \frocc}
    \label{tab:time}
\end{table}

==> sections/table_performance.tex <==
\begin{table}
    \resizebox{\columnwidth}{!}{
        \begin{tabular}{c cc cc cc cc cc cc cc cc}
            \toprule
            \multirow{2}{*}{ID} & \multicolumn{2}{c}{OC-SVM} & \multicolumn{2}{c}{IsoForest} & \multicolumn{2}{c}{Deep SVDD} & \multicolumn{2}{c}{Auto Encoder} & \multicolumn{2}{c}{\frocc}                                                                                                                                                    \\
            \cmidrule(lr){2-3}             \cmidrule(lr){4-5}                \cmidrule(lr){6-7}                \cmidrule(lr){8-9}                   \cmidrule(lr){10-11}
                                & ROC                        & P@n                           & ROC                           & P@n                              & ROC                         & P@n                         & ROC                       & P@n                       & ROC                         & P@n                         \\
            \midrule
            1                   & 98.99 \(\pm\) 0.00         & 92.34 \(\pm\) 0.00            & 98.86 \(\pm\) 0.00            & 91.65 \(\pm\) 0.00               & 97.04 \(\pm\) 0.00          & \emph{93.25 \(\pm\) 0.00}   & \emph{99.38 \(\pm\) 0.00} & 74.32 \(\pm\) 0.00        & \textbf{99.61 \(\pm\) 0.00} & \textbf{99.80 \(\pm\) 0.00} \\
            2                   & \emph{90.21 \(\pm\) 0.00}  & \textbf{88.32 \(\pm\) 0.00}   & 70.83 \(\pm\) 0.00            & 72.83 \(\pm\) 0.00               & 72.70 \(\pm\) 0.00          & \emph{82.70 \(\pm\) 0.00}   & 62.38 \(\pm\) 0.00        & 65.90 \(\pm\) 0.00        & \textbf{92.46 \(\pm\) 0.00} & 79.34 \(\pm\) 0.00          \\
            3                   & 52.21 \(\pm\) 0.00         & 50.02 \(\pm\) 0.00            & 51.47 \(\pm\) 0.00            & 51.42 \(\pm\) 0.00               & \emph{59.32 \(\pm\) 0.00}   & \emph{57.32 \(\pm\) 0.00}   & 56.73 \(\pm\) 0.00        & 51.63 \(\pm\) 0.00        & \textbf{61.93 \(\pm\) 0.00} & \textbf{57.92 \(\pm\) 0.00} \\
            4                   & 49.62 \(\pm\) 0.00         & 50.08 \(\pm\) 0.00            & 54.13 \(\pm\) 0.00            & 50.13 \(\pm\) 0.00               & \emph{67.81 \(\pm\) 0.00}   & \emph{55.21 \(\pm\) 0.00}   & 55.73 \(\pm\) 0.00        & 53.40 \(\pm\) 0.00        & \textbf{71.04 \(\pm\) 0.00} & \textbf{55.62 \(\pm\) 0.00} \\
            5                   & 63.55 \(\pm\) 0.00         & 61.63 \(\pm\) 0.00            & 61.23 \(\pm\) 0.00            & 59.13 \(\pm\) 0.00               & \textbf{71.88 \(\pm\) 0.00} & \textbf{69.38 \(\pm\) 0.00} & 66.73 \(\pm\) 0.00        & \emph{64.71 \(\pm\) 0.00} & \emph{67.12 \(\pm\) 0.00}   & 62.46 \(\pm\) 0.00          \\
            6                   & 54.22 \(\pm\) 0.00         & 61.05 \(\pm\) 0.00            & \textbf{81.21 \(\pm\) 0.00}   & \textbf{79.77 \(\pm\) 0.00}      & \emph{78.21 \(\pm\) 0.00}   & \emph{78.32 \(\pm\) 0.00}   & 56.27 \(\pm\) 0.00        & 66.17 \(\pm\) 0.00        & 69.32 \(\pm\) 0.00          & 71.91 \(\pm\) 0.00          \\
            7                   & 68.12 \(\pm\) 0.00         & 78.17 \(\pm\) 0.00            & \textbf{77.09 \(\pm\) 0.00}   & \textbf{87.09 \(\pm\) 0.00}      & 61.39 \(\pm\) 0.00          & 72.23 \(\pm\) 0.00          & \emph{75.96 \(\pm\) 0.00} & 78.19 \(\pm\) 0.00        & 72.30 \(\pm\) 0.00          & \emph{84.31 \(\pm\) 0.00}   \\
            8                   & 73.51 \(\pm\) 0.00         & 74.22 \(\pm\) 0.00            & \emph{83.19 \(\pm\) 0.00}     & \emph{81.94 \(\pm\) 0.00}        & 68.36 \(\pm\) 0.00          & 68.36 \(\pm\) 0.00          & 76.42 \(\pm\) 0.00        & 76.42 \(\pm\) 0.00        & \textbf{85.14 \(\pm\) 0.00} & \textbf{89.21 \(\pm\) 0.00} \\
            9                   & 53.35 \(\pm\) 0.00         & 59.72 \(\pm\) 0.00            & 63.48 \(\pm\) 0.00            & 61.64 \(\pm\) 0.00               & \textbf{73.24 \(\pm\) 0.00} & \emph{72.74 \(\pm\) 0.00}   & 62.43 \(\pm\) 0.00        & 63.54 \(\pm\) 0.00        & \emph{73.18 \(\pm\) 0.00}   & \textbf{72.83 \(\pm\) 0.00} \\
            10                  & 57.93 \(\pm\) 0.00         & 63.21 \(\pm\) 0.00            & \textbf{85.10 \(\pm\) 0.00}   & \emph{82.83 \(\pm\) 0.00}        & 56.95 \(\pm\) 0.00          & 60.03 \(\pm\) 0.00          & 59.43 \(\pm\) 0.00        & 57.73 \(\pm\) 0.00        & \emph{83.57 \(\pm\) 0.00}   & \textbf{85.91 \(\pm\) 0.00} \\
            11                  & 86.01 \(\pm\) 0.00         & 81.35 \(\pm\) 0.00            & 80.05 \(\pm\) 0.00            & \textbf{87.24 \(\pm\) 0.00}      & \emph{84.73 \(\pm\) 0.00}   & 81.21 \(\pm\) 0.00          & 79.23 \(\pm\) 0.00        & 72.94 \(\pm\) 0.00        & \textbf{86.64 \(\pm\) 0.00} & \emph{83.21 \(\pm\) 0.00}   \\
            \bottomrule
        \end{tabular}
    }
    \caption{Area under the ROC curve and Precision@n scores. ID corresponds to the dataset ID in Table~\ref{tab:data}. For each dataset, \(n\) is the number of positive examples in the test set of that dataset.}
    \label{tab:performance}
\end{table}

==> sections/table_time.tex <==
\begin{table}
    \resizebox{\columnwidth}{!}{
        \begin{tabular}{ccccccccccc}
            \toprule
            \multirow{2}{*}{ID} & \multicolumn{2}{c}{OC-SVM} & \multicolumn{2}{c}{IsoForest} & \multicolumn{2}{c}{Deep SVDD} & \multicolumn{2}{c}{Auto Encoder} & \multicolumn{2}{c}{\frocc}                                                                            \\
            \cmidrule(lr){2-3}             \cmidrule(lr){4-5}                \cmidrule(lr){6-7}                \cmidrule(lr){8-9}                   \cmidrule(lr){10-11}
                                & Train                      & Test                          & Train                         & Test                             & Train                      & Test  & Train & Test  & Train                            & Test          \\
            \midrule
            A1                  & 18.21                      & 1.16                          & \emph{1}\textsuperscript{3}   & \emph{1}                         & 26.03                      & 26.06 & 11.23 & 11.13 & \textbf{0.90}\textsuperscript{1} & \textbf{0.90} \\
            A2                  & 17.66                      & 1.18                          & \emph{1}\textsuperscript{1}   & \emph{1}                         & 25.88                      & 26.00 & 11.79 & 11.35 & \textbf{0.75}\textsuperscript{3} & \textbf{0.93} \\
            A3                  & 10.00                      & 1.19                          & \emph{1}\textsuperscript{1}   & \emph{1}                         & 25.76                      & 25.96 & 12.19 & 11.48 & \textbf{0.78}\textsuperscript{3} & \textbf{0.93} \\
            A4                  & 15.55                      & 1.15                          & \emph{1}\textsuperscript{1}   & \emph{1}                         & 26.09                      & 26.09 & 11.03 & 11.03 & \textbf{0.84}\textsuperscript{2} & \textbf{0.91} \\
            \midrule
            B1                  & 13.51                      & 1.17                          & \emph{1}\textsuperscript{2}   & \emph{1}                         & 25.96                      & 26.03 & 11.48 & 11.23 & \textbf{0.93}\textsuperscript{1} & \textbf{0.92} \\
            B2                  & 23.41                      & 1.91                          & \emph{1}\textsuperscript{4}   & \emph{1}                         & 28.65                      & 26.41 & 16.21 & 12.76 & \textbf{0.56}\textsuperscript{2} & \textbf{0.85} \\
            B3                  & 10.11                      & 1.26                          & \emph{1}\textsuperscript{4}   & \emph{1}                         & 23.50                      & 25.69 & 20.17 & 12.44 & \textbf{0.77}\textsuperscript{1} & \textbf{0.87} \\
            B4                  & 10.14                      & 1.22                          & \emph{1}\textsuperscript{5}   & \emph{1}                         & 25.08                      & 25.82 & 14.58 & 11.98 & \textbf{0.72}\textsuperscript{1} & \textbf{0.91} \\
            B5                  & 10.01                      & 1.21                          & \emph{1}\textsuperscript{4}   & \emph{1}                         & 25.40                      & 25.88 & 13.47 & 11.79 & \textbf{0.73}\textsuperscript{1} & \textbf{0.92} \\
            B6                  & 10.23                      & 1.20                          & \emph{1}\textsuperscript{5}   & \emph{1}                         & 25.61                      & 25.92 & 12.72 & 11.63 & \textbf{0.74}\textsuperscript{2} & \textbf{0.92} \\
            B7                  & 10.02                      & 1.24                          & \emph{1}\textsuperscript{4}   & \emph{1}                         & 24.56                      & 25.76 & 16.44 & 12.19 & \textbf{0.69}\textsuperscript{1} & \textbf{0.90} \\
            \bottomrule
        \end{tabular}
    }
    \caption{Training and test speedups for baselines and \frocc. The speedup is calculated relative to the fastest baseline method, i.e. IsolationForest. A number below 1 indicates the method is faster than the fastest baseline. Lower is better. Superscript shows the rank of the methods based on ROC-AUC scores for the two fastest methods.}
    \label{tab:time}
\end{table}
